THOI: An efficient and accessible library for computing higher-order interactions enhanced by batch-processing

Complex systems are characterized by nonlinear dynamics, multi-level interactions, and emergent collective behaviors. Traditional analyses that focus solely on pairwise interactions often oversimplify these systems, neglecting the higher-order interactions critical for understanding their full collective dynamics. Recent advances in multivariate information theory provide a principled framework for quantifying these higher-order interactions, capturing key properties such as redundancy, synergy, shared randomness, and collective constraints. However, two major challenges persist: accurately estimating joint entropies and addressing the combinatorial explosion of interacting terms. To overcome these challenges, we introduce THOI (Torch-based High-Order Interactions), a novel, accessible, and efficient Python library for computing high-order interactions in continuous-valued systems. THOI leverages the well-established Gaussian copula method for joint entropy estimation, combined with state-of-the-art batch and parallel processing techniques to optimize performance across CPU, GPU, and TPU environments. Our results demonstrate that THOI significantly outperforms existing tools in terms of speed and scalability. For larger systems, where exhaustive analysis is computationally impractical, THOI integrates optimization strategies that make higher-order interaction analysis feasible. We validate THOI accuracy using synthetic datasets with parametrically controlled interactions and further illustrate its utility by analyzing fMRI data from human subjects in wakeful resting states and under deep anesthesia. Finally, we analyzed over 900 real-world and synthetic datasets, establishing a comprehensive framework for applying higher-order interaction (HOI) analysis in complex systems.

==> backup_abstract.tex <==
% Version inicial 23-05-24
%Neuronal networks within the brain represent highly complex, nonlinear dynamical systems characterized by intricate interactions and emergent patterns that challenge traditional linear analyses. Current approaches to quantify such complexity often fall short due to the limitations inherent in model-based measures, necessitating alternative methodologies that can encompass both linear and nonlinear dynamics across multiple organizational levels. This paper introduces THOI, a novel Python library designed to estimate higher order interactions (HOI) within continuous multivariate data through the application of the O-information. Leveraging a Gaussian copula approach for entropy estimation, THOI transforms data into rank-based normal distributions, enabling the computation of entropies and O-information via matrix operations on submatrices of the covariance matrix, optimized for performance on CPU, GPU, and TPU environments. We provide a detailed exposition of the mathematical foundations of O-information, its estimation under Gaussian assumptions, and the efficiencies achieved through batch processing and parallel computation. Comparative analysis against existing tools demonstrates THOI’s computational efficiency and the robustness of its estimative capabilities, marking a significant advancement in the use of the O information measure and its applications to neuroscience research.

% Version Ruben 23-05-24
%Complex systems exhibit nonlinear, intricate, and emergent patterns of interactions that pose significant challenges to traditional linear analysis. While conventional approaches often focus on pairwise interactions, this simplification overlooks higher-order interactions and collective behaviors that are crucial to understanding the full dynamics of such complex systems. Limiting analysis to pairwise interactions fails to capture the multi-dimensional dependencies and emergent properties that arise from the interaction of multiple components, thereby providing an incomplete picture of system behavior. 
%However, these alternatives are usually computationally expensive, hindering widespread scientific applications. Here we present THOI --Torch-based High Order Interactions--, a novel and computationally efficient Python library designed to measure higher-order interactions in continuous multivariate data. % by estimating the O-information. The O-information is a generalized version of the mutual information that informs about the balance between synergy and redundancy in higher-order interactions. 
%By leveraging the Gaussian copula approach for joint entropy estimation, THOI enables the efficient computation of the O-information via matrix operations optimized for performance on CPU, GPU, and TPU environments. We introduce the O-information, its estimation via Gaussian assumptions, and the efficiency achieved through batch processing and parallel computation. Comparative analysis against existing tools demonstrates THOI’s computational efficiency and the robustness of its capabilities. This work opens the access to a widespread application of the O-information and multivariate information theory in science. 


% Version Lao 04-10-24
% Understanding the dynamics of complex systems requires identifying higher-order interactions that go beyond pairwise dependencies, as these multi-dimensional interactions often drive emergent behaviors. Traditional linear analysis, limited to pairwise interactions, overlooks these effects, resulting in an incomplete view of system behavior. The O-information measure, an established technique for capturing multi-way dependencies and estimating joint entropy, becomes computationally expensive when applied to all combinations of higher-order interactions, limiting its practical use in large-scale analyses.
% To address this challenge, we introduce THOI—Torch-based High Order Interactions—a novel, computationally efficient Python library that accelerates the computation of O-information. THOI leverages Gaussian copulas for joint entropy estimation and employs PyTorch’s optimized matrix operations, including batch processing and parallel computation, for efficient execution on CPU, GPU, and TPU environments. This significantly reduces the computational cost and time required, making it feasible to analyze large datasets and explore the complex interactions within multivariate systems.
% We validate THOI against existing tools, demonstrating substantial improvements in speed and scalability without compromising accuracy. Our results show that THOI outperforms current methods, enabling the study of higher-order interactions that were previously computationally prohibitive. We also showcase THOI’s application in a case study analyzing sleep stages through electroencephalography (EEG) data, characterizing higher-order interactions between brain regions in both electrode and source spaces via source localization.
% THOI is open-source and readily available, facilitating the broader application of multivariate information theory in complex system analysis and advancing the study of emergent behaviors across scientific fields.



% Propuesta Rodriigo 27/11/2024
Complex systems are characterized by nonlinear dynamics, multi-level interactions, and emergent collective behaviors. Traditional analyses that focus solely on pairwise interactions often oversimplify these systems, neglecting the higher-order interactions that are critical to understanding their full collective dynamics. Recent advances in multivariate information theory offer a principled framework for quantifying these higher-order interactions, capturing key properties such as redundancy, synergy, shared randomness, and collective constraints. However, two major challenges remain: the accurate estimation of joint entropies and the combinatorial explosion of interacting terms. To address these challenges, we introduce THOI (Torch-based High-Order Interactions), a novel, efficient Python library designed to compute high-order interactions in continuous-valued systems. THOI leverages the well-established Gaussian copula method for joint entropy estimation, coupled with state-of-the-art batch and parallel processing techniques to optimize performance across CPU, GPU, and TPU environments. We demonstrate that THOI significantly outperforms existing tools in terms of speed and scalability, without sacrificing accuracy. In particular, THOI reduces the time required to exhaustively analyze all interactions in a system of 30 variables to 6 hours. For larger systems, where exhaustive analysis is computationally impractical, THOI incorporates optimization strategies that make higher-order interaction analysis feasible. We validate THOI's accuracy using synthetic datasets with parametrically controlled interactions and further demonstrate its utility by analyzing fMRI data from human subjects in both a wakeful resting state and under deep anesthesia.


%Complex systems typically display nonlinear dynamics, intricate interactions across multiple organizational levels, and emergent collective behaviors. Focusing solely on pairwise interactions can significantly limit our understanding of those systems, as it neglects higher-order interactions and the full spectrum of interdependencies implicated in collective behavior. This reductionist view can result in an incomplete or misleading representation of the underlying dynamics. Recent advances in multivariate information theory --where Shannon's entropy is a key metric-- provide a principled way to quantify these higher-order interactions and to also identify their quality in terms of shared randomness, collective contrains, redundancy and synergy. However, this approach implies two major technical obstacles: the estimation of joint entropies and the combinatorial explosion.
% To address these challenges, we present THOI (Torch-based High Order Interactions), a novel, ready-to-use and computationally efficient Python library that accelerates the computation of high-order interactions for continous valued systems. THOI leverages the established Gaussian copulas approach for joint entropy estimation and leverage state-of-the-art batch and parallel processing techniques for efficient execution on CPU, GPU, and TPU environments. This innovation reduces the time required to exhaustively analyze interactions in a system of 30 variables from over 200 days to less than 24 hours. For larger systems where the exhaustive approach becomes infeasible, THOI incorporates optimization strategies.



%This significantly improves computational time, making it feasible to analyze exhaustively all the combinations of a system of 30 variables in less than 1 day, whereas previous implementation would take more than 200 days. We also implemented optimization algorithms for cases where the exhaustive approach becomes infeasible. We validated the accuracy of our implementation with synthetic systems where high-order interactions, synergy and redundancy can be parametrically controlled. Finally, we demonstrat its use with neuroimaging and electroencephalographic data of humans undergoing anaesthesia and different sleep stages, respectively.


% large datasets and explore the complex interactions within multivariate systems.
% propuesta de thoi, leveraging gaussian copula y batch processing. the first allows to estimate all the measure based solely in the covariance matrix while the second allows an efficient computation of all hois, leveraging GPU and TPU architecture. Our results show that THOI outperforms current methods in terms of computational time and accuracy, enabling the study of higher-order interactions that were previously computationally prohibitive. We also leverage our efficient implementation to develop optimization algrithms for cases wheren the exahsutive approach is not feasible. Finally, we demonstrate its use on source localized sleep EEG data.
